Adaptive Repetitions Strategies in IEEE 802.11bd

A new backward compatible WiFi amendment is under development by the IEEE bd Task Group towards the so-called IEEE 802.11bd, which includes the possibility to transmit up to three repetitions of the same packet. This feature increases time diversity and enables the use of maximum ratio combining (MRC) at the receiver to improve the probability of correct decoding. In this work, we first investigate the packet repetition feature and analyze how it looses its efficacy increasing the traffic as an higher number of transmissions may augment the channel load and collision probability. Then, we propose two strategies for adaptively selecting the number of transmissions leveraging on an adapted version of the channel busy ratio (CBR), which is measured at the transmitter and is an indicator of the channel load. The proposed strategies are validated through network-level simulations that account for both the acquisition and decoding processes. Results show that the proposed strategies ensure that devices use optimal settings under variable traffic conditions.

==> Source files ArXiv June 2022/Acronyms.tex <==
\begin{acronym} 
\acro{3GPP}{Third Generation Partnership Project}
\acro{2D}{two-dimensional}
\acro{2G}{second generation}
\acro{3G}{third generation}
\acro{4G}{fourth generation}
\acro{5G}{fifth generation}
\acro{6G}{sixth generation}
\acro{5GAA}{5G Automotive Association}
\acro{5GS}{5G system}
\acro{AF}{application function}
\acro{AIFS}{arbitration inter-frame space}
\acro{AMC}{adaptive modulation and coding}
\acro{AoI}{age of information}
\acro{AS}{application server}
\acro{AWGN}{additive white Gaussian noise}
\acro{BEP}{beacon error probability}
\acro{BM-SC}{Broadcast Multicast Service Center}
\acro{BP}{beacon periodicity}
\acro{B-CSA}{broadcast \ac{CSA}}
%\acro{BR}{beacon resource}
%\acro{BRF}{\ac{BR}-frequency}
%\acro{BRT}{\ac{BR}-time}
\acro{BSM}{basic safety message}
\acro{BSS}{basic service set}
\acro{BS}{base station}
\acro{C-ITS}{cooperative-intelligent transport systems}
\acro{C-NOMA}{Cooperative \ac{NOMA}}
\acro{C-V2X}{cellular-\ac{V2X}}
\acro{CA}{collision avoidance}
\acro{CAM}{cooperative awareness message}
\acro{CAV}{connected and autonomous vehicle}
\acro{CBR}{channel busy ratio}
\acro{CCDF}{complementary cumulative distribution function}
\acro{CDF}{cumulative distribution function}
\acro{CDMA}{code-division multiple access}
\acro{CoMP}{coordinated multi-point}
\acro{CN}{core network}
%\acro{CP-OFDM}{cyclic prefix \ac{OFDM}}
\acro{CP}{cyclic prefix}
\acro{CP-OFDM}{cyclic prefix orthogonal frequency-division multiplexing}
\acro{CPM}{collective perception message}
\acro{CR}{channel occupancy ratio}
\acro{CRDSA}{contention resolution diversity slotted ALOHA}
\acro{CSA}{coded-slotted ALOHA}
\acro{CSD}{cyclic shift diversity}
\acro{CSI}{channel state information}
\acro{CSIT}{channel state information at the transmitter}
\acro{CSIR}{channel state information at the receiver}
\acro{CSMA/CA}{carrier sense multiple access with collision avoidance}
\acro{CSSR}{candidate single-subframe resource}
\acro{D2D}{device-to-device}
\acro{DCC}{decentralized congestion control}
\acro{DCF}{distributed coordination function}
\acro{DCI}{downlink control
information}
\acro{DCM}{dual carrier modulation}
\acro{DENM}{decentralized environmental notification message}
\acro{DMRS}{demodulation reference signal}
\acro{DRX}{discontinuous reception}
\acro{DSRC}{dedicated short range communication}
\acro{DOT}{Department of Transportation}
\acro{EC}{European Commission}
\acro{ECP}{extended cyclic prefix}
\acro{EDCA}{enhanced distributed coordination access}
\acro{EDGE}{Enhanced Data rates for GSM Evolution}
\acro{eMBMS}{evolved Multicast Broadcast Multimedia Service}
\acro{eMMB}{enhanced mobile broadband}
\acro{eNodeB}{evolved NodeB}
\acro{EPC}{Evolved Packet Core}
\acro{EPS}{Evolved Packet System}
\acro{ETSI}{European Telecommunications Standards Institute}
\acro{eV2X}{enhanced V2X}
\acro{FCC}{Federal Communications Commission}
\acro{FCD}{floating car data}
\acro{FD}{in-band full-duplex}
\acro{FDD}{frequency division duplex}
\acro{FDMA}{frequency division multiple access}
\acro{FEC}{forward error correction}
\acro{FR1}{frequency range 1}
\acro{FR2}{frequency range 2}
\acro{GNSS}{global navigation satellite system}
\acro{GPRS}{general packet radio service }
\acro{GPS}{global positioning system}
\acro{HARQ}{hybrid automatic repeat request}
\acro{HD}{half-duplex}
\acro{HSDPA}{High Speed Downlink Packet Access}
\acro{HSPA}{High Speed Packet Access}
\acro{IBE}{in-band emission}
\acro{ICI}{Inter-carrier interference}
\acro{IDMA}{interleave-division multiple access}
\acro{IM}{index modulation}
\acro{IP}{Internet Protocol}
\acro{IPG}{inter-packet gap}
\acro{IR}{incremental redundancy}
\acro{ISI}{inter-symbol interference}
\acro{ITS}{intelligent transport system}
\acro{i.i.d.}{independent identically distributed}
\acro{KPI}{key performance indicator}  
\acro{LDPC}{low-density parity-check}
\acro{LDS}{low-density spreading}
\acro{LIDAR}{light detection and ranging}
\acro{LOS}{line-of-sight}
\acro{LTE}{long term evolution}  
\acro{LTE-D2D}{\ac{LTE} with \ac{D2D} communications}  
\acro{LTE-V2X}{long-term-evolution-vehicle-to-anything} \acro{LTE-V2V}{\ac{LTE}-\ac{V2V}}
\acro{MAC}{medium access control}
\acro{MBMS}{Multicast Broadcast Multimedia Service}
\acro{MBMS-GW}{MBMS Gateway}
\acro{MBSFN}{MBMS Single Frequency Network}
\acro{MCE}{Multi-cell Coordination Entity}
\acro{MEC}{mobile edge computing}
\acro{MCM}{maneuver coordination message}
\acro{MCS}{modulation and coding scheme}
\acro{MIMO}{multiple input multiple output}
\acro{ML}{machine learning}
\acro{MRC}{maximum ratio combining}
\acro{MRD}{maximum reuse distance}
\acro{MUD}{multi-user detection}
\acro{NEF}{network exposure function}
\acro{NGV}{Next Generation V2X}
\acro{NHTSA}{National Highway Traffic Safety Administration}
\acro{NLOS}{non-line-of-sight}
\acro{NOMA}{non-orthogonal multiple access}
\acro{NOMA-MCD}{\ac{NOMA}-mixed centralized/distributed}
\acro{NR}{new radio}
\acro{OBU}{on-board unit}
%\acro{OCB}{outside of the context of a \ac{BSS}}
\acro{OCB}{outside of the context of a basic service set}
\acro{OEM}{Original equipment manufacturer}
\acro{OFDM}{orthogonal frequency-division multiplexing}
\acro{OFDMA}{orthogonal frequency-division multiple access}
\acro{OMA}{orthogonal multiple access}
\acro{OTFS}{orthogonal time frequency space}
\acro{pdf}{probability density function}
\acro{PAPR}{peak to average power ratio}
\acro{PCF}{policy control function}
\acro{PCM}{platoon control message}
\acro{PD}{packet delay}
\acro{PEP}{pairwise error probability} 
\acro{PER}{packet error rate}
\acro{PIAT}{packet inter-arrival time}
\acro{PRB}{physical resource block}
\acro{PSCCH}{Physical Sidelink Control Channel}
\acro{PSFCH}{Physical Sidelink Feedback channel}
\acro{PSSCH}{Physical Sidelink Shared channel}
\acro{PHY}{physical}
\acro{PL}{path loss}
\acro{PLMN}{Public Land Mobile Network}
\acro{PPPP}{ProSe Per-Packet Priority}
\acro{PPPR}{ProSe Per-Packet Reliability}
\acro{ProSe}{Proximity-based Services}
\acro{PRR}{packet reception ratio}
\acro{QAM}{quadrature amplitude modulation}
%\acro{QC-LDPC}{quasi-cyclic low-density parity-check}
\acro{QC-LDPC}{quasi-cyclic \ac{LDPC}}
\acro{QoS}{quality of service}
\acro{QPSK}{quadrature phase shift keying}
\acro{RAN}{Radio Access Network}
\acro{RAT}{radio access technology}
%\acro{RB}{resource block}
%\acro{RBP}{resource block pair}
\acro{RF}{radio frequency}
\acro{RIS}{reconfigurable intelligent  surface}
\acro{RL}{reinforcement learning}
\acro{RR}{radio resource}
\acro{RRC}{radio resource control}
\acro{RRI}{resource reservation interval}
\acro{RSRP}{reference signal received power}
\acro{RSSI}{Received Signal Strength Indicator}
\acro{RSU}{road side unit} 
\acro{SAE}{Society of Automotive Engineers}
\acro{SAI}{Service Area Identifier}
\acro{SB-SPS}{sensing-based semi-persistent scheduling}
\acro{SC-FDMA}{single carrier frequency division multiple access}
\acro{SC-PTM}{Single Cell Point To Multipoint}
\acro{SCS}{subcarrier spacing}
\acro{SCMA}{sparse-code multiple access}
\acro{SI}{self-interference}
\acro{SIC}{successive interference cancellation}
\acro{SIFS}{short inter-frame space}
\acro{S-UE}{scheduling UE}
\acro{SCI}{sidelink control information}
\acro{SDN}{Software-defined networking}
\acro{SFFT}{symplectic finite Fourier transform}
\acro{SHINE}{simulation platform for heterogeneous interworking networks}
\acro{SINR}{signal-to-interference-plus-noise ratio}
\acro{SNR}{signal-to-noise ratio}
%\acro{SPS}{semi-persistent scheduling} % REPLACED BY SB-SPS
\acro{SRS}{sounding reference signal}
\acro{STBC}{space time block codes}
\acro{SV}{smart vehicle}
\acro{TB}{transport block}
\acro{TBC}{time before change}
\acro{TBE}{time before evaluation}
\acro{TDD}{time-division duplex}
\acro{TDMA}{time-division multiple access}
\acro{TR}{technical report}
\acro{TS}{technical specification}
\acro{TTI}{transmission time interval}
\acro{UAV}{unmanned aerial vehicle}
\acro{UD}{Update delay}
%\acro{UE}{user equipment}
\acro{PSDU}{Physical Layer Convergence 
Protocol Service 
Data Unit}
\acro{UMTS}{universal mobile telecommunications system}
\acro{URLLC}{ultra-reliable and ultra-low latency communications}
\acro{USIM}{Universal Subscriber Identity Module}
\acro{UTDOA}{uplink time difference of arrival}
\acro{V2C}{vehicle-to-cellular} 
\acro{V2N}{vehicle-to-network}
\acro{V2I}{vehicle-to-infrastructure} 
\acro{V2P}{vehicle-to-pedestrian}
\acro{V2R}{vehicle-to-roadside}
\acro{V2V}{vehicle-to-vehicle} 
\acro{V2X}{Vehicle-to-everything} 
\acro{VAM}{VRU awareness message}
\acro{VRU}{vulnerable road user}
\acro{VUE}{vehicular user equipment}
\acro{WAVE}{wireless access in vehicular environment}
\acro{WBSP}{wireless blind spot probability}
\acro{PPDU}{physical layer protocol data unit}
\acro{LLR}{log-likelihood ratio}
\end{acronym}



==> Source files ArXiv June 2022/TableSettings.tex <==
\begin{table*}[!t]
\caption{Main simulation parameters and settings%\hl{Vincent: it is not fully clear from Table 1, what is the sensitivity figure or SINR for PSDU data}
\vspace{-2mm}
\label{Tab:Settings}}
\footnotesize
%\scriptsize
\centering
\begin{tabular}{p{2.5cm}p{14cm}}
\hline \hline
\emph{\textbf{Scenario}} & Highway, 3+3 lanes, variable vehicle density, average speed 120 km/h with 12 km/h std. deviation\\
%\hline
\emph{\textbf{Data traffic}} & 350~bytes packets generated every 100 ms \\
%\hline
\emph{\textbf{MAC settings}} & Maximum contention window 15, AIFS 110 $\mu s$, SIFS 32 $\mu s$\\%, maximum 3 repetitions\\
\emph{\textbf{MCS}} & MCS 2 (QPSK, CR$=0.5$), with error rate probability based on the curves in \cite{BazZanIoaMar:C20} (1~dB @ PER=0.5)\\
\emph{\textbf{Rx thresholds}} & For preamble detection -100~dBm, for unknown signals -65~dBm, for the CBR evaluation -85~dBm\\ 
%\hline
\emph{\textbf{Channel and power}} & Single 10 MHz channel at 5.9~GHz, tx power 23 dBm (not including antenna gain), antenna gain 3~dBi, noise figure 6~dB\\
\emph{\textbf{Propagation}} & WINNER+ Scenario B1 propagation model, correlated shadowing with 3~dB variance and decorr. dist. 25~m \\
%\footnote{The value of -98 dBm, which is in agreement with what obtained in off-the shelf devices, corresponds to a \ac{SNR} of 0 dB with a noise figure of 6 dB. } \\ 
%\hline
%\emph{\textbf{Repetitions}} & \\
%Number of repetitions $\Ntx$ & 0, 1, 2, 3\\
\hline \hline
\end{tabular}
%\vskip -0.4cm
\end{table*}


==> Source files ArXiv June 2022/TableSettingsLarge.tex <==
\begin{table}[!t]
\caption{Main simulation parameters and settings%\hl{Vincent: it is not fully clear from Table 1, what is the sensitivity figure or SINR for PSDU data}
\vspace{-2mm}
\label{Tab:Settings}}
\footnotesize
%\scriptsize
\centering
\begin{tabular}{p{4cm}p{3cm}}
\hline \hline
\emph{\textbf{Scenario}} & \\
Road layout & Highway, 3+3 lanes\\%, 4 m width \\
Vehicle density $\density$ & Variable\\
Average speed & 140 km/h \\
Speed std. deviation & 14 km/h\\

\hline
\emph{\textbf{Power and propagation}} & \\
Channel & 5.9~GHz (ITS band) \\
Bandwidth & 10 MHz \\
Transmission power density & 23 dBm\\ %13~dBm/MHz \\
Antenna gain (tx and rx)  & 3~dBi \\
Noise figure & 6~dB \\
Propagation model & WINNER+, Scenario B1 \\
Shadowing & Variance 3~dB, decorr. dist. 25~m \\

\hline
\emph{\textbf{Data traffic}}& \\
Packet generation & 10~Hz \\ 
Packet size $S_\text{p}$ & 350~bytes \\ 

\hline
\emph{\textbf{Access layer settings}} & \\
MCS & 2 (QPSK, CR$=0.5$)\\
Maximum contention window & 15\\
AIFS & 110 $\mu s$\\
SIFS & 32 $\mu s$\\
Error rate probability & \ac{SINR}-based curves in \cite{BazZanIoaMar:C20}, 1~dB @ PER=0.5\\
Sensing thr. for preamble & -100~dBm\\
Sensing thr. for unknown signals & -65~dBm\\
Sensing thr. for the CBR evaluation & -85~dBm\\ 
%\footnote{The value of -98 dBm, which is in agreement with what obtained in off-the shelf devices, corresponds to a \ac{SNR} of 0 dB with a noise figure of 6 dB. } \\ 
\hline
\emph{\textbf{Repetitions}} & \\
Number of repetitions $\Ntx$ & 0, 1, 2, 3\\
\hline \hline
\end{tabular}
%\vskip -0.4cm
\end{table}


==> TableSettingsLarge.tex <==
\begin{table}[!t]
\caption{Main simulation parameters and settings%\hl{Vincent: it is not fully clear from Table 1, what is the sensitivity figure or SINR for PSDU data}
\vspace{-2mm}
\label{Tab:Settings}}
\footnotesize
%\scriptsize
\centering
\begin{tabular}{p{4cm}p{3cm}}
\hline \hline
\emph{\textbf{Scenario}} & \\
Road layout & Highway, 3+3 lanes\\%, 4 m width \\
Vehicle density $\density$ & Variable\\
Average speed & 140 km/h \\
Speed std. deviation & 14 km/h\\

\hline
\emph{\textbf{Power and propagation}} & \\
Channel & 5.9~GHz (ITS band) \\
Bandwidth & 10 MHz \\
Transmission power density & 23 dBm\\ %13~dBm/MHz \\
Antenna gain (tx and rx)  & 3~dBi \\
Noise figure & 6~dB \\
Propagation model & WINNER+, Scenario B1 \\
Shadowing & Variance 3~dB, decorr. dist. 25~m \\

\hline
\emph{\textbf{Data traffic}}& \\
Packet generation & 10~Hz \\ 
Packet size $S_\text{p}$ & 350~bytes \\ 

\hline
\emph{\textbf{Access layer settings}} & \\
MCS & 2 (QPSK, CR$=0.5$)\\
Maximum contention window & 15\\
AIFS & 110 $\mu s$\\
SIFS & 32 $\mu s$\\
Error rate probability & \ac{SINR}-based curves in \cite{BazZanIoaMar:C20}, 1~dB @ PER=0.5\\
Sensing thr. for preamble & -100~dBm\\
Sensing thr. for unknown signals & -65~dBm\\
Sensing thr. for the CBR evaluation & -85~dBm\\ 
%\footnote{The value of -98 dBm, which is in agreement with what obtained in off-the shelf devices, corresponds to a \ac{SNR} of 0 dB with a noise figure of 6 dB. } \\ 
\hline
\emph{\textbf{Repetitions}} & \\
Number of repetitions $\Ntx$ & 0, 1, 2, 3\\
\hline \hline
\end{tabular}
%\vskip -0.4cm
\end{table}

